Towards Understanding and Applying Security Assurance Cases for Automotive Systems

Security Assurance Cases (SAC) are structured bodies of arguments and evidence used to reason about security properties of a certain artefact. SAC are gaining focus in the automotive domain as the need for security assurance is growing due to software becoming a main part of vehicles. Market demands for new services and products in the domain require connectivity, and hence, raise security concerns. Regulators and standardisation bodies started recently to require a structured for security assurance of products in the automotive domain, and automotive companies started, hence, to study ways to create and maintain these cases, as well as adopting them in their current way of working. In order to facilitate the adoption of SAC in the automotive domain, we created CASCADE, an approach for creating SAC which have integrated quality assurance and are compliant with the requirements of ISO/SAE-21434, the upcoming cybersecurity standard for automotive systems. CASCADE was created by conducting design science research study in two iterative cycles. The design decisions of CASCADE are based on insights from a qualitative research study which includes a workshop, a survey, and one-to-one interviews, done in collaboration with our industrial partners about the needs and drivers of work in SAC in industry, and a systematic literature review in which we identified gaps between the industrial needs and the state of the art. The evaluation of CASCADE was done with help of security experts from a large automotive OEM. It showed that CASCADE is suitable for integration in industrial product development processes. Additionally, our results show that the elements of CASCADE align well with respect to the way of working at the company, and has the potential to scale to cover the requirements and needs of the company with its large organization and complex products

==> TexFiles/paperA/backup.tex <==
\iffalse
\paragraph{Interview 1} was conducted with two interviewees, to tackle two of the usage scenarios, as explained in the methodology \todo{refer to the section where this is mentioned}.
The interviewees were one solution manager, and one solution train engineer, both from Company B, and the two usage scenarios discussed are US3 \emph{''As a project manager, I would use SAC to make sure that a project is ready from a security point of view to be closed and shipped to production.''}, and US6 \emph{''As a product owner, I would use SAC to make an assessment of the quality of my product from a security perspective, and make a road-map for future security development.''}
The interviewees said that today, the security assurance in projects is mostly based on experience, and is done by providing evidence such as test reports for some claims. These claims are derived from projects' requirements are not put together in a structured way. the interviewees also stressed that what is done today is simply not sufficient given the rapid evolution of connectivity in the vehicles. Historically there has been \emph{''a trust in the physical shell (the cab) around the items in the vehicle.''}, but today these items are connected to the outside world, and can be a target for cyber attacks.
 
As per the interviewees, having SACs as a part of scoping projects, setting the milestones and deliverables, and connecting them to the development process, would be of great value to security assurance from a project management perspective. Additionally from a product point of view, having a holistic SAC which is updated by the related projects would give the product owner an understanding of how secure the product is at different time-points, e.g., after integrating changes from different projects.

Both interviewees agreed that SACs should be built on a product level rather than a project level. SACs should be integrated and built within project, but only to contribute towards the product's SAC, especially that the majority of the projects are delta projects, i.e., make changes to an existing system. A product, however, may be big and complex, and may include items that are more interesting from a security perspective than others, e.g., Electrical Control Units (ECU) that are connected to the outside world in a vehicle. In this case there needs to be a severity assessment to focus on the right items.

The interviewees think that the SAC work can be integrated into the project manager's and product owner's work by captured it in projects' requirements. The interviewees emphasize that it is important to work on quality, e.g., security as a part of the development process, and not as a separate activity. The workload in the beginning will be high, but with time, there will be patterns that can be reused to build SAC with less effort.

When it comes to the challenges, the interviewee consider handling the complexity of the product (vehicle in this case), and finding right competences to be the main ones. Additionally, there has to be a decision from upper management and an agreement from the teams to work wit SAC, which is also a challenge. On the other hand, the interviewees consider working with SAC \emph{''an opportunity for the company to build a reputation of building secure vehicles.'' } 


\paragraph{Interview 2} was conducted with a functional safety assessor in Company B, with a wide range of experience in compliance. The scenario discussed in the interview was US2 \emph{ As a member of the compliance team, I would use detailed SAC to prove to authorities that the company has complied to a certain standard, legislation,.. etc and show them evidence of my claim of compliance.} 
In the current situation, the compliance team is only concerned with safety matters, as per the interviewee. The only involvement with security issues is when there is a breach which affects the product's safety. There is, however, a need to consider security as \emph{''Security issues can be as serious if not more serious than safety issues, especially that they can affect a multiple vehicles at a time.''} according to the interviewee. The expectation is that SAC can serve as an umbrella document for all the analysis documents. Hence it can be used by an assessor to find related document to assess compliance to a certain standard.

The SAC should be created on a whole vehicle level, as per the interviewee. It needs, however, to be dividable in manageable pieces, i.e., pieces that can be managed by individuals, which would be responsible for the corresponding part of the SAC. For compliance purposes, the authorities look at system level, hence, for every project that includes changes in the system, there us a need to study the impact on other artefacts, which would also cause changes in SAC.

How working with SAC can be integrated within the way of working of the compliance team depends much on SACs are implemented. If they are integrated within the projects (as they should according to the interviewee), then the compliance team would have the responsibility of following them up throughout the project, as well as making sure that they are complete after the verification phase. 

When it comes to the challenges, the interviewee considers the main challenge to be finding resources and competences to carry out the work related to creating, maintaining, assessing and supporting SACs. 

\paragraph{Interview 3} was conducted with a component owner in Company B, who is experienced in purchasing and working with suppliers. The scenario discussed in the interview was US8 \emph{ As a member of the purchase team, I would include SAC as a part of the contracts made with suppliers, in order to have evidence of the fulfillment of security requirements at delivery time, and to track progress during development time.}.
As of today, security assurance when working with suppliers is about making sure of the fulfillment of security requirement, and running test cases on a sample of the requirements. However, \emph{''there is an uncertainty to a large extent that the received software is secure''}, as per the interviewee. On the other hand, safety critical functions, e.g., breaking, is handled differently. The suppliers are usually asked to show how requirements are broken down and implemented during regular review sessions. In some cases, suppliers were asked to provide safety cases, which were used together with the internal safety cases to make sure that the claims align. The interviewee expects that SAC can be used in the same manner as safety cases. Additionally, they can be used to communicate with suppliers, to discuss security internally, and as a supporting artifact for creating security requirements.

Regarding the granularity of the cases, the interviewee distinguishes between two types of SAC: the ones created at the supplier's end, and the ones created by the company.
On the supplier's side the cases should be on the ECU level, followed by a threat-based level. Whereas the company-owned SACs should be on the complete vehicle level, and broken down to ECU level, which is contributed by the suppliers. An important aspect mentioned by the interviewee is the weighting of the claims \emph{''The cases should indicate the severity of the claims''}. This is to be able to prioritize the claims during the follow up sessions with the suppliers, and when testing the implementation.


Integrating SAC in the current way of working with suppliers would increase the workload, but there are no obvious conflicts, according to the interviewee. However, there is a need for tools for store, extract, and compare SACs. Additionally, a version handling tool is also required to keep track of the SACs and their changes. The interviewee also mentioned the need to use an exchangeable format when building the cases, on both ends (supplier and company), in order to compare and integrate them.


When it comes to the challenges, the interviewee said that \emph{''An experience from safety is that even when there is education about the cases, it was much more complicated when actual work was done.''}. Hence, there needs to be practical training on SAC in the industrial context. Another challenge mentioned by the interviewee is finding resources with the right competences to carry out the SAC related work.


\paragraph{Interview 4} was conducted with a senior legal counsel at Company B. The scenario discussed in the interview was US12 \emph{ As a legal risk owner, I would use SAC in court if a legal case is raised against the company for security related issues. I would use the SAC to prove that sufficient preventive actions were taken}. In the current situation, the company has not had any legal case for security related issues, but there have been cases claiming that feature malfunctioning have caused accidents. These were all functional safety related according to the interviewee. However, there is an increasing need to make sure that assets, e.g., ECU data, do not suffer from security issues. 

Current evidence used in court for these kinds of legal cases are of two types: \emph{(i)} usage of technology according to an acceptable standard; \emph{(ii)} implementations of the used standards and technologies are correctly done (this should be certified by a third party assessor). Hence, if the ISO 21434 \cite{iso21434} becomes an industry standards, then it can be used as an evidence in court.

When it comes to the expectations of SAC, the interviewee said  that \emph{''an evidence based structured approach to argue about security would definitely be used as evidence in court.''}. However, it is very important to assure the quality of the case when it comes to completeness in the argumentation and evidence, if the case would be used in court. The SAC used as an evidence will be available to the opponents, and it could be exploited to find holes and error to be used against the company.

The granularity needed for the SAC depends pretty much on the legal case according to the interviewee. However, there is a need to create SACs for complete vehicles, and views that could be broken down. This is to avoid cases where a legal case against the company involves a composition of systems (end-to-end function), and SACs are created for a subset of these systems. This would be a weakness if they are used as evidence).

The creation of SACs should, from a company perspective, be during development to assure security, as \emph{''It is unacceptable to release unsecured vehicles''} according to the interviewee. However, from a legal perspective, SACs can be created once a legal case is filed. However, this could lead to questions asking why the SACs were not created during development. Additionally, it would increase the probability of the risk of having insufficient evidence, as it would be harder to locate and assign them. Moreover, from a liability perspective, it is much better to create the SAC proactively.

As per the interviewee, if SACs are to be used as evidence, the relevant stakeholders in the company will be reached out and asked to provide the SACs when needed. Then the legal responsible will have meetings with the stakeholders to understand it. This means that the ownership of the SACs would not be the responsibility of the legal responsible, even if it is created specially for a legal case. The legal responsible would be a user of the SAC.

At the end, the interviewee stressed that introducing a structured way of security assurance \emph{''can lead to creating better systems which can protect the company from issues from regulators and third parties.''}. However, there has to be a buy-in on different levels in the company in order to do this in a correct way.
\fi







\iffalse
The first part of the study revealed a major need for security assurance cases to comply with both current and future standards, best practices, and legislation. Not all of the identified \todo{Find a term for these} standards / legislation / best practices provide an explicit requirement for creating security assurance cases. However, we believe that these cases can be used to address the needs for security assurance in them.


The task of the break-out session proved to be difficult for the participants. This can be due to multiple factors such as the complication and large scope of the task, the groups members being new to each other (never worked together before), and the possible lack of experience of some participants in the specific processes associated with the usage scenarios.

Another observation from the workshop is that answering the who question was the hardest part in the break-out session. The who question was mainly directed towards finding out who would be responsible for the security assurance cases in the different scenarios. It included multiple sub-questions, e.g., who is the owner, maintainer, and other. We believe that this particular question was hard to figure out because it was asked in an industrial organization where people are already fully occupied. Hence, it was hard for the participants to imagine how new activities can be introduced to existing roles. Furthermore, even when the participants were free to suggest new roles for the task, it was still hard for them to figure out where in the organizations these roles should be and how they should be embed in the organizational structure.





TODO: differences, specificities?
Severity should be indicated when SAC is used to talk with suppliers (in order to focus on the important aspects in the control meetings), while in the legal case example, the whole case should be weighted equally.
When working with suppliers, there was an emphasise on having a common language and tool support (very different from other usages). These needs apply to all usages of course, but they are essential for this particular scenario.

When working with suppliers, there is no rules or restrictions from the company's side on how to build the SACs other than the format, i.e., no restrictions on the strategies or evidence to use, or even the granularity level (how fine-grained the claims can be).

Traceability and change analysis was mentioned for compliance (as learned from safety), hence the more mature, the more concerns about quality...
TODO: frequencies and quotes
\fi




\iffalse
\subsubsection{Value:}
All five interviewees believed that security assurance cases can provide value if properly designed. This value comes in the form of a structured, complete, comprehensive and continuous approach to cybersecurity.
When it comes to the current security assurance way of working, one interviewee described it as passive, i.e., the reaction to security threats happens following an incident which affects safety. The other interviewees said that it depends to a large extent on the requirements of the system in question. Additionally, all the interviewees stressed that it is hard, or even almost impossible, as of today to have a complete picture of the status of cybersecurity for a given product.
Regarding the expectation of security assurance cases, the interviewees mentioned multiple possible usages. These include: \emph{(i)} provide a view on what the current status and risks of the product are cybersecurity related, \emph{(ii)} provide a common understanding of the product security by different stakeholders, e.g., OEM, and suppliers, in a given project,\emph{(iii)} provide an easy way in for new employees to understand how cybersecurity is argued for and handled in the company, \emph{(iv)} as an evidence to be used in legal cases, especially to claim state of the art development processes and techniques when it comes to cybersecurity.

\subsubsection{Content and Structure:}
There was a consensus among the interviewees that security assurance cases shall be based on complete products and not temporarily product updates (projects). However, such a generic case might not be useful to all the stakeholders, or applicable to all usage scenarios. Thus, the cases have to be built in a way that makes them flexible on the abstraction level. Moreover, there must be support for different viewpoints of the cases, i.e., the users should be able to get a holistic view, and to zoom in a specific part of the case when more details are required. 
When asked about the desired approach for creating the argumentation part of the case, the interviewees preferred a conventional top-down approach. However, two of the interviewees believed that a bottom-up approach can be beneficial especially when creating cases for existing systems. Hence, a mixed approach starting from top-down and then integrate bottom-up approaches made sense when thinking about different contexts. 
In order to create a complete case on product level, the work must be possible to divide into smaller work packages that later can be integrated to give the holistic view. The structure must also consider different authorities view on what parts requiring certification etc. A tool for handling the case would be beneficial also to provide version handling. A security case approach shall support that it is in some cases relates to a vehicle function and in other cases a system or component. The structure must also be considered when interfacing assurance cases from OEM with different suppliers.

\subsubsection{Integration:}
The assurance case shall follow the way of working. Whether there should be any specific role handling the assurance case or not, or several roles/teams shall take this responsibility, differs among the interviewed persons. The security case needs to be possible to update regularly. A security expert team might be necessary to support the work, at least in the beginning. If people believes that the security case improves quality, it will be easier to integrate it into the traditional work.

\subsubsection{Challenges:}
A truck is a complex product to build a security case for. Top management must support the introduction of security cases in the organization. Who will do the work? Where shall the work be stored and how can it be easily updated when necessary? The organization must avoid that the assurance case becomes yet another paper work, but instead provides something of real value to as many stakeholders as possible!
\fi

==> TexFiles/paperA/breakout.tex <==
The usage scenarios selected for the break-out session were US3, US6, and US12.


\begin{table}
	\begin{center}
		\begin{tabular}{p{2cm}p{6cm}}

		
			\\       \textbf{Question}
	        & \textbf{Answer}

			\\ \midrule
			                      What&Compliance with the company's cybersecurity standard 
			\\ \midrule
			                      Who& Owner: Project manager
			                      \\ & For: Product Owner
			                      \\ & Contributors: Project team, train
			                      \\& QA: Verification team
			                      \\& Maintenance: Line organization
			  \\ \midrule
			                      When&Start: Early project phase
			                      \\ &Evolves: Change related
			                      \\ & Changes: Wrong assumptions, change requests, bugs.
			                      \\ &Finish: Release gate
			\\ \midrule
			                      How&Evidence: Risk assessments verification reports, review reports.
			\\ \midrule
			                      Challenges& Dependencies and support                      
			\\ \bottomrule
		\end{tabular}
		\caption{Summary of the discussion in the break-out session about US3}
		\label{res_bo_1}
	\end{center}
\end{table}

\paragraph{US3} Table \ref{res_bo_1} shows the answers provided by the team which worked on US3. The participants decided that the scope of the case from this US is the same as an internal project's scope. This was then used to answer the questions in the exercise. The only claim suggested by the team is a high level one for complying with the company's security standard. When it comes to the roles, the participants suggested that the project manager should be the owner of the case, and that the project team would contribute towards creating and verifying it. The case should be then handed to the owner of the product in which the project took place for integrating it with the product's case. The life-cycle of the case starts in an early phase of the project as per the team. However, they did not specify a particular phase. The case then evolves as the project evolves, and finishes when the project is released, after it serves its main goal in the decision making of releasing the project. The team suggest multiple sources for evidence, such as risk assessment, review, and verification reports. The main challenge pointed out by the team are managing and tracing dependencies between the claims of this case and claims of other projects, as well as the claims of the product's case. A second challenge is to provide the support needed to work with security assurance cases, both when it comes to competences and tools.

\begin{table}
	\begin{center}
		\begin{tabular}{p{2cm}p{6cm}}

		
			\\       \textbf{Question}
	        & \textbf{Answer}

			\\ \midrule
			                      What&Following standards and industry best practices
			                      \\& Legal compliance, e.g., GDPR
			                      \\& Fulfillment of security attributes
			\\ \midrule
			                      Who& Owner: Product owner
			                      \\ & Contributors: product team, security team
			                      \\& QA: Product owner
			                      \\& Maintenance: Product owner
			  \\ \midrule
			                      When&Start: Concept study phase
			\\ \bottomrule
		\end{tabular}
		\caption{Summary of the discussion in the break-out session about US6}
		\label{res_bo_2}
	\end{center}
\end{table}

\paragraph{US6} Table \ref{res_bo_2} shows the answers provided by the team which worked on US6. The team members were not able to set a clear scope of the case of this US as it depends heavily on the product in question. Hence, it was difficult for them to answer many of the questions in the exercise. The main claims suggested by the team were about complying with standards and regulations, as well as the fulfillment of security attributes, such as confidentiality, integrity, and availability. When it comes to the \emph{who} question, the team had a very hard time finding out who the tasks associated with SAC should be assigned to. At the end, they decided that the product owner for which the SAC is created, should also own the SAC, be responsible of its quality assurance, and maintenance. Other contributors according to the team are the product team for creating the case, and the security team for support. The last question partially answered by the team was the \emph{when} question, and the suggestion was to start building the SAC in a very early stage at the product development phase, namely the concept study phase. However, the team did not discuss creating SAC for an existing product.

\begin{table}
	\begin{center}
		\begin{tabular}{p{2cm}p{6cm}}

		
			\\       \textbf{Question}
	        & \textbf{Answer}

			\\ \midrule
			                      What&Claims that sufficient measures have been taken
			\\ \midrule
			                      Who& Owner: Lawyer, task manager, investigation leader.
			                      \\ & For: Upper management, court
			                      \\ & Contributors: SMEs, product owner
			                      \\& QA: Lawyers, external security experts
			                      \\& Maintenance: Product owner
			  \\ \midrule
			                      When&Start: At start of court case ( assuming that the SAC is already created for a certain project or product)
			                      \\ &Evolves: As evidence are being collected
			                      \\ & Changes: As evidence are being added.
			                      \\ &Finish: When the court case is closed
			\\ \midrule
			                      How&Evidence: TARA, verification and validation reports, and risk mitigation documentation
			\\ \midrule
			                      Challenges&Traceability needs to be improved (for the documents used in SAC)
			                      \\&Roles and ownership identification
			\\ \bottomrule
		\end{tabular}
		\caption{Summary of the discussion in the break-out session about US12}
		\label{res_bo_3}
	\end{center}
\end{table}

\paragraph{US12} Table \ref{res_bo_3} shows the the results of the break out session's exercise for US12. The participants considered the SAC related to this US to be limited to the legal case. This means that the SAC would be created (or extracted fro another SAC) only when needed. This is when a legal case is filed against the company for security related issues. The main goal of this SAC is showing that sufficient security measures have been taken for the system / component in question, according to the participants. When it comes to the roles, the participants suggested multiple owners for the SAC, e.g., the lawyer responsible for the legal case, or investigation leader. The creation of the SAC would be contributed by the product owner and the Subject Matter Experts of the product in question, and the quality assurance would be the responsibility of the users of the case, i.e., the lawyers, with help from external security experts. When it comes to maintaining the SAC, the team suggested that the product owner should take on that task, as it would be a part of a generic one for the product. The life-cycle of this SAC according to the team follows the life-cycle of the legal case, meaning that the SAC is created at the start of the legal case, evolves as the legal case evolves, and finishes when the legal case is closed. The participants also suggested evidence for the SAC, e.g., Threat Analysis and Risk Assessment (TARA) reports, verification results, and risk mitigation documents. The team considered traceability for the relevant documents of the SAC to be a major challenge in addition to organisational challenges in identifying the right roles for SAC related tasks.

TODO: summary, etc...

To summarize, we got th
It is clear that even though we got answers on questions, we still needed to dig deeper into the US as in many cases, the participants were not confident in their answers. For example in US12, the team answered all the who questions, but still mentioned a challenge to identify the roles when SAC will be applied in the company. 

==> TexFiles/paperC/BU.tex <==
mapping of different architectural views and diagrams to elements of the asset-based SAC:

1. The domain view of the system which shows the boundaries and high level interactions can be used in asset identification. At this level the identified assets would also be in a high level.

2. The component diagram (structural view) and class diagram (implementation view) can both contribute towards decomposing the assets. This de-composition can be based on the different parts of the assets that are used by different components, or based on an assessment of the assets' sensitivity levels.

3. For tracing the assets, the following diagrams can be used: 
- Deployment diagram (physical view) can be used to trace the assets to their "at rest" states (where the assets are stored).
- Deployment diagram + component diagram can be used to trace the assets to the "in use" state (while the asset is being used/processed/transformed... etc)
- Sequence diagrams (behavioural view) can be used for the "in transition" state traceability of assets. This is because we can find information regarding how the data is being transferred between different components using calls. Additionally, the deployment diagram can be used at this point to see if the asset is being transferred between different physical devices (which would probably require different/additional security mechanisms to assure security).

4. When it comes to the evidence, the component diagram and the deployment diagram can reveal much information of the architectural styles/patterns/tactics used in the system, hence they can be used to derive evidence. For example, if the system uses the heartbeat tactic, that can be used as evidence for  availability.





For hardware assets. -> deployment.
4+1 views: UC to describe requirements
Evidence: more than what we have. (tim maybe)





The first step is to identify the assets of the system.



When we want to decompose the asset, we look into how it can be used. If parts of the asset will be used in different functions / by different components (this is for setting the abstraction level)  

Also different sensitivity levels.


In the breaking down of the asset with regards to traceability we look into the components that hold/use these assets. 


This step should be done after the architecture is completed. We look for the structural view in the architecture to see the relationship between the components. 

The transition of a card information would be 1) from a customer to the card reader machine 2) from the machine to the system 3) from the system to the external bank system

Evidence: security domains are identified and assigned to every potential attacker in every interface interface.

-----------------------



-----------------------

Reflection after applying the CoCoME case:

If we are going to claim that we are providing quality assurance in our approach, we have to consider multiple things:

1. The quality assurance completeness claims, e.g., "All and only relevant assets are identified" seem to be more like assumptions. It would be very hard to assign evidence to back this kinds of claim up. 
- Using a technique or systematic approach) to find that the assets are identified.
- Using a standard or process (to reason that it is enough)... etc


2. There is no measurement that can be applied to the completeness nor the confidence claims. 

3. Traceability links, e.e., to responsible people/roles are also important for QA. For example if we argue that we have non-repudiation in an asset and we provide evidence that we use audit logs, then there has to be someone responsible to audit these logs. If that person leaves, then the evidence becomes obsolete.



Maybe we can add attributes to the claims and evidence. Examples are: responsible persons and time for service. In the latter, we can examine whether evidence still hold. An example would be: A new technology has been developed which makes computers much faster. Is our encryption key length sufficient? Another example would be just to add new evidence.

- how we use a case not only as a document, but also as an activity / process to be used in the company.


Other concerns:
1. The CIA are not sufficient. An example is non-repudiation, and privacy.
2. When it comes to the hardware assets, I believe it would take part of the asset decomposition and asset traceability strategies.
3. Having the argument over security properties above asset decomposition (and maybe also over asset identification) is not impossible... however, it is not as intuitive.
4. Not all the strategies in the approach are always applicable, and also not necessarily in the order we suggest. Hence it could be interesting to have more than 2 blocks. Then when applying, the user can choose which blocks to use (maybe also it could be used multiple times)



What are assets in automotive? 
How are they decomposed.
Take a look at the asset list of the automotive company.


Physical/Hardware Resources
ECU (hardware), Sensors, Actuators, Mechanical Components, GPS
Software 
ECU (software), libraries, OS, virtualization
Network and Communication
Controller Area Network (CAN), Local Interconnect Network (LIN), Media Oriented Systems Transport (MOST), FlexRay, Automotive Ethernet, Mobile Network, IoT, WiFi, Bluetooth
Information and Data
User Data and Information, Logs, Events.





Example is that traceability might now be applicable if we have hardware assets. 
Maybe we can have building blocks (lego blocks) to build the case. 
Maybe the company is mature and has clear requirements of security properties from the beginning, then they can start with that.

Question: where does the vulnerability analysis come into play?


==> TexFiles/paperC/extended_approach.tex <==
Asset-first / asset-driven approach:
%A suggest we call it asset-driven as it starts with assets
The approach consists of blocks which in turn consists of levels.
Each block is governed by a mindset while each level consists of one or more levels of strategies. 
Each strategy is connected to at least one context, which in turn is connected to quality assurance claims.
Each block is 
The approach consists of the following blocks:


Top claim: Here we need to discuss the abstraction level of that claim
For now, we say that the top claim is about having adequate security for a specific "item".
The item might be a complete product, a system, a user function, or a component. This depends on both the complexity of the item, and the needs for the case from the applying organization (we have seen in a previous study that there are many usage scenarios for SAC, and some of them require claims on a certain abstraction level.


Generic arguments: these are argument applicable for a larger context than the item of the top claim.
These arguments contain claims about for example the cybersecurity culture in the company, compliance to certain standards, and the application of a certain security ensuring process. 
These claims are usually valid not only for the item in question, but usually to a set of items within the organization.
In that case, these claims can be reused for all SACs within that organization.


white hat block: 

This is the top block of the approach. To create the arguments in this block, we need to have the mindset of someone who wants to protect the item.

Here we have three (or maybe two) levels: 
1. Asset level: Here is basically everything we originally had in the asset-based approach.
    This is done to make sure that we know what is valuable in the item, i.e., what we want to protect.
    
2. Damage scenarios: when we have identified the assets and their traceability, we identify damage scenarios for that asset. The corresponding claims at the end would be a negation of the possibility of that damage scenario.
(a possibility here is to think about risks instead of damage scenarios..)
 
3. Security goals: this is where we claim that the assets we identify are secure from the damage scenarios. Here, we can define these in different stages of the product life-cycle, e.g., security goals in the design, implementation, and maintenance.

Black-hat block:
Two levels:
1. Threat scenario: what are the possible threat scenarios that might compromise the identified security goals? The claims would be that a certain scenario is not possible (or maybe does not have a significant impact).
2. Attack path: what are the possible attack paths for the identified threat scenarios?


Resolver block
Here we have two levels:
1. What are the requirements for preventing the attack from happening?
2. What evidence do we have that the requirement is fulfilled.







General rules: 

At each level, there has to be an evaluation to see if I would like to go further

If I am able to provide sufficient evidence at any level, I would stop.

It is essential to be able to reuse some of the arguments in different parts of the cases (and of course in different cases). For that, we see how important it is to have tool support (automation) for creating the cases. 

If we base the SAC on user functions, we will get claims that are redundant throughout the SAC. This should be solved by reusing and creating views (a view where the claim is mentioned whenever applicable, and another with only references).

Abstraction level (for views) can be set on a sub-SAC level. We can create multiple levels, and then assign the sub-SAC to one of these. The visualization of the SAC will be based on that. However, this may lead to gaps, so there must be a method to assure validity / satisfyability when we do that. (here we have to transform the SAC into a logical expression).


What do we need a tool for?
- We need to identify the notation to be used for creating the cases. 
    Are we going to use CAE, GSN, or a modified version of some of them.
- Based on the notation, we need to identify the meta-model (what elements and relations we have).
- We need to have a database where we can store the items of the cases, and their relationships.
- We need a tool to assist in the creation of the cases (if we decide to have visual cases, we don't want to spend a lot of time trying to draw the elements in a different tool. The tool has to be integrated with the database.
- The tool needs to be integrated to other tools (e.g., system engineering) in order to create traceability useful for e.g., for maintainability.
- Automatically transform the case (or a view of it) into a logical formula, and check its validity






Örjan:

Takes the architects hat.
Think about attackers (owner / internal vs outsider / external)



==> TexFiles/paperC/leftover.tex <==
\section{Asset-based Approach}\label{sec:app}

\begin{figure*}
\begin{center}
  \includegraphics[width=1\linewidth]{Images/Asset-Centric.png}
\end{center}
        \caption{The asset-centric approach for creating security assurance cases} 
        \label{fig:assetApproach}
\end{figure*}
%What are assets
In general terms, assets are artifacts of interest to a certain entity. In computer security, these artifacts can be data, software, or hardware. The importance of assets makes them the target for attackers. 

The asset-centric approach for creating security assurance cases takes into consideration the importance of assets to organizations. Hence, it builds the argumentation by putting assets in the center of focus, with a goal to show that these assets are secure from cyber security attacks. By doing that, we will also prove that the system or product in question is secure.

An important design principle in the asset-cerntric approach is the structuring of the quality assurance of the case. This is done by arguing over the completeness and confidence in the case along with the argumentation structure. Each level of argumentation is associated with at least one claim about completeness, and each level of evidence is associated with at least one claim for confidence. A similar concept is used by Hawkins et al. \cite{safetyConfidence} to argue about the confidence of safety cases. 


\subsection{Argumentation}
The argumentation in the asset-centric approach consists of two main blocks, as shown in figure \ref{fig:assetApproach}
\paragraph{High-level block}
The high-level block contains the top claim, and the first level of argumentation. If mapped to an asset analysis done in an OEM, the abstraction of this level corresponds to the level between a conceptual user function, and the concrete software/hardware asset levels. At this level of analysis, the company knows exactly what the functions of the vehicle are, and how they should work (as functional requirements are known), but they do not know how the implementation would look like. Hence, the context of this level is the asset identification technique. 

As examples of asset identification techniques in an automotive OEM we list the following:
\begin{itemize}
    \item Finding assets in the vehicle’s different HW components.
    \item Finding assets in different states of the vehicle (moving state, parking state… etc)
    \item Finding assets in requirements (safety requirements with security implication for instance).
\end{itemize}

\paragraph{Low-level block}
%% Asset traceability to hardware.
%which process activities are related to the assets.
%asset types -> activities
The low level block can consist of multiple levels. If mapped to an asset analysis done in an OEM, the abstraction of this level corresponds to a low level asset analysis. In this level, the company knows more details about the implementation. The structure of this block varies depending on the nature of the assets found in the previous block. The different variations could be based for example on one or more of the following variants:
\begin{itemize}
    \item Asset id: what assets exist and are identified.
    \item Asset relations: the relationships among the assets, e.g. dependability.
    \item Asset traceability (where the assets are). For example:
        \begin{itemize}
            \item While asset is “at rest”. This is when the asset is stored, e.g. in the storage unit of an ECU.
            \item While asset is “on the move”. This is when the asset is in transition between two entities. For example when a sensor data is being transferred from the sensor to an ECU.
            \item While asset is “in use”. This is when the asset is being used. For example when some diagnostics data is being processed at a backend system.
        \end{itemize}
    \item Asset type (signals, user data… etc). This also indicates whether the asset would have implication on the local part of the vehicle (one ECU), or on a bigger part of the vehicle (multiple ECUs).
    \item Asset security properties, e.g. CIA.
\end{itemize}


\subsection{Completeness}
We use the term completeness as a quality assurance term which refers to the level of coverage of the claims in each level of the SAC.
We determine a level in the security assurance case by the strategy used to decompose the claims. Each level in the case has one strategy. If a claim afterwards is decomposed using a different strategy, then we consider this to be a different level.

In each level of argumentation, we add at least one completeness claim that refines the strategy used in that level. The role of this claim is to make sure that the strategy covers all and only the relevant claims in the argumentation level.
The completeness is also related to the context of the argumentation strategy. It is where we find the information needed to determine if the completeness claim is fulfilled or not.

\subsection{Confidence}
We use the term confidence as a quality assurance term which indicates the level of certainty that a claim is fulfilled based on the provided evidence.
This quality assurance attribute is used in each level of a security assurance case where at least one claim is justified by evidence. The confidence attribute is expressed as a claim, which takes the form: "The evidence provided for claim/claims X make an acceptable level of confidence". What makes an acceptable level of confidence shall be defined in the context of the strategy. The confidence claim itself must be justified by evidence of course.

-------------------------
\subsection{Ideas}

\subsection{Application}
\subsubsection{Information sources}
In order to obtain the necessary information needed to create a SAC using the asset-based approach, we need to look at different views of the architecture of the system in question. In this section, we provide a mapping between different architecture views and the levels of the asset-based SAC. The views we look into are the 4+1 identified by Kruchen \cite{kruchen} 

\begin{itemize}
    \item Identification of assets: The scenarios view is an abstract view of the important requirements. It is usually illustrated by use cases. It can be used to determine system boundaries and high-level interactions. Hence, it can be used to identify assets on an abstract level. Another source of information at this level is the physical view which can be used to identify hardware assets.
    \item Decomposition of assets: The development view can contribute towards the decomposition of the abstract assets obtained from the scenarios view. An example is the use of a component diagram to determine how a high-level asset is distributed among different components. Another example is to decompose based on an assessment of the assets' sensitivity levels.
    \item Traceability of assets: For tracing the assets, the physical view can be used for the "at rest" state, i.e., finding information on where the assets are stored. Additionally, the development view and the physical view together can be used to trace the assets in the "in-use" state, which refers to the assets being used, processed or transformed. The last traceability state we have is the "in-transition" state. The views which can be used for this state are: \emph{(i) the logical view} to determine relations and dependencies among components/classes related to the asset, \emph{(ii) the process view} which can be represented by sequence and communication diagrams. This view is important to trace the behaviour of the components that use the assets, and how they interact,  \emph{(iii) the physical view} which allows to tracing the transition of an asset between physical devices (which would probably require different/additional security mechanisms to assure security).
    \item Evidence: all the views can be used to collect evidence. For example, the component diagram (development view) and the deployment diagram (physical view) can reveal much information of the architectural styles/patterns/tactics used in the system, hence they can be used to derive evidence, e.g., if the system uses the heartbeat tactic, that can be used as evidence for availability.
\end{itemize}

\subsection{Building blocks}
%Definition of a block
We consider each part of an argument consisting of a strategy and sub-claims connected to it to be a block. Hence, as shown in Figure \ref{fig:assetApproach} \todo{update the figure to show all the blocks}, we have four blocks in the abstracted template of an asset-based SAC. 
%composability
There are two main reasons for us to believe that a SAC built using the asset-based approach should use composable blocks
\begin{itemize}
    \item Not all the blocks are needed in all cases. For instance, a company might be mature when it comes to its asset analysis, and decide to jump directly to the detailed assets block without going through the asset identification one.
    \item The order of the blocks varies among cases. Some companies might be mature when it comes to cyber-security and decide to start the argumentation with the security properties' block. 
\end{itemize}
 
Each of these blocks should have a quality assurance sub-block connected to it. 

In addition to these blocks, there might be some generic argumentation about security that would be applicable to the whole case rather than a specific claim. An example is to argue that the processes applied by the company are up to security standards. This argument applies to every case, and every block. Hence, we consider this to be a vertical argument that supports the case as a whole.


Riccardo: Not all process-related claims have to be on the side.. some would be related to the product.
Find examples where it makes sense to compose in different ways.

Evidence: show how they can be in different branches.. (not on the same level as leaves)

By next week: clarify the idea of composability.
viewification: how it would look like in practice.
maybe we need a TIM MORE SPECIFIC TO ASSETS.


\todo{Suggestion: combine the asset identification and decomposition blocks.. and describe that one block might have multiple levels.}
\subsection{Views}
%what is meant by views
We learned in a previous study that it is important to have different views of a SAC in order for different stakeholders to use it. This becomes even more important in large organizations, where stakeholders with different roles might use the SACs differently. Examples of these views are: \emph{(i)} an abstract view showing a SAC for a vehicle based on its main end-user functionality, which can be used by upper management or sales force; \emph{(ii)} a fine grained view that can be used by a product owner to make a go/no-go decision on shipping an update on an ECU software. 
%what is needed
The asset-based approach focuses on the assets for creating the SAC, but it is also important to provide other views as well. This means that the case shall incorporate all the information needed to provide these views.
%How to achieve that (extremely hard) (this needs a tool!)
While creating the SAC, there has to be traceability links to important models and development artefacts. This means that when an asset is identified, we also need to identify the functions and processes associated with that asset.


Riccardo: What are the views, and what are the requirements.
Views: end-function, process oriented (vcc). 
What requirements are there to provide these views.

Security about asset protection: from a security pov it makes sense to start from here.. but in practice it could be different (side activity where functions are thought of)
Driver for SAC: not only from a user pov, but also from a security perspective.


Is the case stronger to start from assets and go towards other views (less assumptions, or more specific to the product). Compare to literature is an option.


Exercises: try things out and then compare and show why AB is better (if it is).

Sync with JP. Mail: today we discussed this and we would like to sync..







\subsection{The CoCoME case}
In the top block, and in order to identify the assets, we have to look closely into the domain and the requirements. In the example of a supermarket, we know that the customers usually use their credit cards to purchase, hence this information must be secure. 

If we are going to claim that we are providing quality assurance in our approach, we have to consider multiple things:

1. The quality assurance completeness claims, e.g., "All and only relevant assets are identified" seem to be more like assumptions. It would be very hard to assign evidence to back this kinds of claim up. 
- Using a technique or systematic approach) to find that the assets are identified.
- Using a standard or process (to reason that it is enough)... etc


2. There is no measurement that can be applied to the completeness nor the confidence claims. 

3. Traceability links, e.e., to responsible people/roles are also important for QA. For example if we argue that we have non-repudiation in an asset and we provide evidence that we use audit logs, then there has to be someone responsible to audit these logs. If that person leaves, then the evidence becomes obsolete.



Maybe we can add attributes to the claims and evidence. Examples are: responsible persons and time for service. In the latter, we can examine whether evidence still hold. An example would be: A new technology has been developed which makes computers much faster. Is our encryption key length sufficient? Another example would be just to add new evidence.

- how we use a case not only as a document, but also as an activity / process to be used in the company.


Other concerns:
1. The CIA are not sufficient. An example is non-repudiation, and privacy.
2. When it comes to the hardware assets, I believe it would take part of the asset decomposition and asset traceability strategies.
3. Having the argument over security properties above asset decomposition (and maybe also over asset identification) is not impossible... however, it is not as intuitive.
4. Not all the strategies in the approach are always applicable, and also not necessarily in the order we suggest. Hence it could be interesting to have more than 2 blocks. Then when applying, the user can choose which blocks to use (maybe also it could be used multiple times)



\subsection{An automotive case}

We tested the approach on a complete vehicle product.
In the top level, we claimed the the vehicle is acceptably secure.
We then identified the main assets of a vehicle. This identification was based on a domain analysis.

What are assets in automotive? 
How are they decomposed.
Take a look at the asset list of the automotive company.


Physical/Hardware Resources
ECU (hardware), Sensors, Actuators, Mechanical Components, GPS
Software 
ECU (software), libraries, OS, virtualization
Network and Communication
Controller Area Network (CAN), Local Interconnect Network (LIN), Media Oriented Systems Transport (MOST), FlexRay, Automotive Ethernet, Mobile Network, IoT, WiFi, Bluetooth
Information and Data
User Data and Information, Logs, Events.


Q: is an end-to-end function also an asset? in this case, many of the assets identified in the first level intersect (data assets, ecu software, ecu hardware... etc)



-------------------------

The headlight example:
The asset identification is part of the risk analysis in the concept phase.



\subsection{The CoCoME case}
In the CoCoME case, the assets are well identified, which makes it possible for us to implement a party of our approach, which is the white-hat part. However, the threats and attack paths are not identified, which makes creating the rest of the case require manual extraction of these based on the identified assets and a suggested threat model (e.g., STRIDE). 
When it comes to the resolver block, the case provides requirements on how to protect the system's assets by defining security domains, and assigning the interfaces of the system to these domains. 
Some evidence can be extracted from the case, however, these are not as concrete as we would like them to be in order to establish confidence in the SAC. 
Since the case covers one system and is not in the context of an organization, it is not possible to extract generic arguments for reuse. Similarly, it lacks the context elements.

Identification of potential attackers is covered in the case, and gave us insight of how to integrate this point into our approach.



In the top block, and in order to identify the assets, we have to look closely into the domain and the requirements. In the example of a supermarket, we know that the customers usually use their credit cards to purchase, hence this information must be secure. 

If we are going to claim that we are providing quality assurance in our approach, we have to consider multiple things:

1. The quality assurance completeness claims, e.g., "All and only relevant assets are identified" seem to be more like assumptions. It would be very hard to assign evidence to back this kinds of claim up. 
- Using a technique or systematic approach) to find that the assets are identified.
- Using a standard or process (to reason that it is enough)... etc


2. There is no measurement that can be applied to the completeness nor the confidence claims. 

3. Traceability links, e.e., to responsible people/roles are also important for QA. For example if we argue that we have non-repudiation in an asset and we provide evidence that we use audit logs, then there has to be someone responsible to audit these logs. If that person leaves, then the evidence becomes obsolete.



Maybe we can add attributes to the claims and evidence. Examples are: responsible persons and time for service. In the latter, we can examine whether evidence still hold. An example would be: A new technology has been developed which makes computers much faster. Is our encryption key length sufficient? Another example would be just to add new evidence.

- how we use a case not only as a document, but also as an activity / process to be used in the company.


Other concerns:
1. The CIA are not sufficient. An example is non-repudiation, and privacy.
2. When it comes to the hardware assets, I believe it would take part of the asset decomposition and asset traceability strategies.
3. Having the argument over security properties above asset decomposition (and maybe also over asset identification) is not impossible... however, it is not as intuitive.
4. Not all the strategies in the approach are always applicable, and also not necessarily in the order we suggest. Hence it could be interesting to have more than 2 blocks. Then when applying, the user can choose which blocks to use (maybe also it could be used multiple times)



\subsection{Ideas}

\subsection{Application}
\subsubsection{Information sources}
In order to obtain the necessary information needed to create a SAC using the asset-based approach, we need to look at different views of the architecture of the system in question. In this section, we provide a mapping between different architecture views and the levels of the asset-based SAC. The views we look into are the 4+1 identified by Kruchen \cite{kruchen} 

\begin{itemize}
    \item Identification of assets: The scenarios view is an abstract view of the important requirements. It is usually illustrated by use cases. It can be used to determine system boundaries and high-level interactions. Hence, it can be used to identify assets on an abstract level. Another source of information at this level is the physical view which can be used to identify hardware assets.
    \item Decomposition of assets: The development view can contribute towards the decomposition of the abstract assets obtained from the scenarios view. An example is the use of a component diagram to determine how a high-level asset is distributed among different components. Another example is to decompose based on an assessment of the assets' sensitivity levels.
    \item Traceability of assets: For tracing the assets, the physical view can be used for the "at rest" state, i.e., finding information on where the assets are stored. Additionally, the development view and the physical view together can be used to trace the assets in the "in-use" state, which refers to the assets being used, processed or transformed. The last traceability state we have is the "in-transition" state. The views which can be used for this state are: \emph{(i) the logical view} to determine relations and dependencies among components/classes related to the asset, \emph{(ii) the process view} which can be represented by sequence and communication diagrams. This view is important to trace the behaviour of the components that use the assets, and how they interact,  \emph{(iii) the physical view} which allows to tracing the transition of an asset between physical devices (which would probably require different/additional security mechanisms to assure security).
    \item Evidence: all the views can be used to collect evidence. For example, the component diagram (development view) and the deployment diagram (physical view) can reveal much information of the architectural styles/patterns/tactics used in the system, hence they can be used to derive evidence, e.g., if the system uses the heartbeat tactic, that can be used as evidence for availability.
\end{itemize}

\subsection{Building blocks}
%Definition of a block
We consider each part of an argument consisting of a strategy and sub-claims connected to it to be a block. Hence, as shown in Figure \ref{fig:assetApproach} \todo{update the figure to show all the blocks}, we have four blocks in the abstracted template of an asset-based SAC. 
%composability
There are two main reasons for us to believe that a SAC built using the asset-based approach should use composable blocks
\begin{itemize}
    \item Not all the blocks are needed in all cases. For instance, a company might be mature when it comes to its asset analysis, and decide to jump directly to the detailed assets block without going through the asset identification one.
    \item The order of the blocks varies among cases. Some companies might be mature when it comes to cyber-security and decide to start the argumentation with the security properties' block. 
\end{itemize}
 
Each of these blocks should have a quality assurance sub-block connected to it. 

In addition to these blocks, there might be some generic argumentation about security that would be applicable to the whole case rather than a specific claim. An example is to argue that the processes applied by the company are up to security standards. This argument applies to every case, and every block. Hence, we consider this to be a vertical argument that supports the case as a whole.


Riccardo: Not all process-related claims have to be on the side.. some would be related to the product.
Find examples where it makes sense to compose in different ways.

Evidence: show how they can be in different branches.. (not on the same level as leaves)

By next week: clarify the idea of composability.
viewification: how it would look like in practice.
maybe we need a TIM MORE SPECIFIC TO ASSETS.


\todo{Suggestion: combine the asset identification and decomposition blocks.. and describe that one block might have multiple levels.}
\subsection{Views}
%what is meant by views
We learned in a previous study that it is important to have different views of a SAC in order for different stakeholders to use it. This becomes even more important in large organizations, where stakeholders with different roles might use the SACs differently. Examples of these views are: \emph{(i)} an abstract view showing a SAC for a vehicle based on its main end-user functionality, which can be used by upper management or sales force; \emph{(ii)} a fine grained view that can be used by a product owner to make a go/no-go decision on shipping an update on an ECU software. 
%what is needed
The asset-based approach focuses on the assets for creating the SAC, but it is also important to provide other views as well. This means that the case shall incorporate all the information needed to provide these views.
%How to achieve that (extremely hard) (this needs a tool!)
While creating the SAC, there has to be traceability links to important models and development artefacts. This means that when an asset is identified, we also need to identify the functions and processes associated with that asset.


Riccardo: What are the views, and what are the requirements.
Views: end-function, process oriented (vcc). 
What requirements are there to provide these views.

Security about asset protection: from a security pov it makes sense to start from here.. but in practice it could be different (side activity where functions are thought of)
Driver for SAC: not only from a user pov, but also from a security perspective.


Is the case stronger to start from assets and go towards other views (less assumptions, or more specific to the product). Compare to literature is an option.


Exercises: try things out and then compare and show why AB is better (if it is).

Sync with JP. Mail: today we discussed this and we would like to sync..



%Assets can be found in different layers 
%\begin{itemize}
%    \item Finding assets in the vehicle’s different HW components.
%    \item Finding assets in different states of the vehicle (moving state, parking state… etc)
%    \item Finding assets in requirements (safety requirements with security implication for instance).
%\end{itemize}
%The high-level block contains the top claim, and the first level of argumentation. If mapped to an asset analysis done in an OEM, the abstraction of this level corresponds to the level between a conceptual user function, and the concrete software/hardware asset levels. At this level of analysis, the company knows exactly what the functions of the vehicle are, and how they should work (as functional requirements are known), but they do not know how the implementation would look like. Hence, the context of this level is the asset identification technique. 


%\paragraph{Low-level block}
%% Asset traceability to hardware.
%which process activities are related to the assets.
%asset types -> activities
%The low level block can consist of multiple levels. 





Intro:

Story: We are building a SAC approach which is asset-centric and with built-in quality assurance. We apply the approach on different cases both from industry and online sources. 

Alternative: We are building an approach for a SAC which is derived from ISO 21434. In terms of contribution (difference to literature) we are building-in quality assurance, by extracting requirements from the standard which contribute to building confidence in the case. We also make it easier for practitioners to apply the approach by decomposing the case into main blocks which get populated during different phases of product development. Additionally, we distinguish generic claims which are applicable to the whole company from the ones which are specific to a product. By doing so, we make it possible for practitioners to re-use the generic part for every case. 
We validate the approach by applying it on the example provided in the ISO standard, and verifying it with an automotive company. The verification consists of the following:
- Making sure that we capture the generic claims for later re-use.
- Assessing the confidence in the case provided by the derived QA claims.
- Making sure that the approach is capable of reaching an argumentation level on which evidence can be assigned. (is it leading to actionable claims?)

Örjan: We should identify who would be able to evaluate and assess. 
We can ask some ppl from the verification team to verify that the claims and justifiable.
Christian works on the "review" type of verification which can be used to justify the QA claims

Next meeting: go through the case and give a first assessment by Örjan and then we can see who can proceed.

Afshin will provide us with the HoliSec cases (hopefully)




- Making sure that the flow of the case follows the development phases in the company (concept phase, product development, production, and maintenance)

- Discuss the possibility to extract different views from a SAC to satisfy the needs of different stakeholders.
- Making sure the cases created using the approach satisfy the requirements for cybersecurity cases in the ISO standard.

We start from the standards to create the approach, and then we apply on other two cases from two different companies. 
Three case studies (one from the standard, and then we tested with the other two)


\todo[inline]{pick two or three validation points (actionable pint as one), and how to measure.. strategy to gather the data.}

Sheet 1 and sheet 2 together provide a guidance to how to create the case. (also aligned with ISO)

We are not the first, early work mentioning asset-based in

1) A.C. Goodger, N.H.M. Caldwell, J. T. Knowles
What does the Assurance Case Approach deliver for Critical Information Infrastructure Protection in cybersecurity?
IET International Conference on System Safety, 2012

Asset (and asset analysis) are mentioned as central to assurance cases
Asset - risks - mitigations argumentation strategy
No practical advise on how to

2) Vaise Patu, Shuichiro Yamamoto
Identifying and implementing security patterns for a dependable Security Case
16th International Conference on Computational Science and Engineering, 2013

``Assets and data'' mentioned in the paper (somehow)
Asset analysis mentioned (sec requirements)
See Figure 2: C I A of data (where data as a whole is the asset) - not so deep

Motivation:

Why asset-based:
It is intuitive to start thinking about security assurance from a standpoint which considers what is valuable in the system, i.e., assets. This is also inline with the example of the security standard we reviewed, which starts by identifying asserts. 

Why built-in quality assurance:
Confidence in a SAC is essential for it to be useful. Assurance cases are used to create confidence in a system or product. This is not possible to achieve if we don't have confidence in the SAC itself.  

\smallskip

The rest of the paper is structured as follows. In Section \ref{sec:rw} we discuss the related work. In Section \ref{sec:method} we describe the research questions and the methodology. In Section \ref{sec:app} we present the approach used in this study. In Sections \ref{sec:res} we present the results. Section \ref{sec:end} presents the concluding remarks.



validation:


\subsection{An automotive case}

We tested the approach on a complete vehicle product.
In the top level, we claimed the the vehicle is acceptably secure.
We then identified the main assets of a vehicle. This identification was based on a domain analysis.

What are assets in automotive? 
How are they decomposed.
Take a look at the asset list of the automotive company.


Physical/Hardware Resources
ECU (hardware), Sensors, Actuators, Mechanical Components, GPS
Software 
ECU (software), libraries, OS, virtualization
Network and Communication
Controller Area Network (CAN), Local Interconnect Network (LIN), Media Oriented Systems Transport (MOST), FlexRay, Automotive Ethernet, Mobile Network, IoT, WiFi, Bluetooth
Information and Data
User Data and Information, Logs, Events.


Q: is an end-to-end function also an asset? in this case, many of the assets identified in the first level intersect (data assets, ecu software, ecu hardware... etc)



-------------------------

The headlight example:
The asset identification is part of the risk analysis in the concept phase.





\textbf{Örjan's thoughts}:
In the example, from an AB Volvo perspective, we would consider the vehicle with offboard services, to be the product. The product would be divided down into items, in order to make the analysis feasible. For vehicle onboard parts, we would mainly divide them into EndUserFunctions and I do not know the exact name, but I think we could say that the ISO-21434 Appendix G example would fall into the EnduserFunction "external lighting". 
That is the EnduserFunction "external lighting" would be our item. The next step would then be to perform damage analysis on this item to find the related assets. The assets related to our product (and all items then) might perhaps be generalized into the following categories:
\begin{itemize}
    \item vehicle functionality (the attackers want to use the vehicle or tamper with the vehicle’s functionality for own purpose or impede the rightful user from utilizing the vehicle functionality),
    \item information (the attackers want gain access to sensitive information),
    \item vehicle or parts of the vehicle (the attackers want to steal the vehicle or expensive parts), services (similar to vehicle functionality?), 
    \item brand (the attackers want to discredit the brand and/or credit themselves). In order to simplify the asset identification, we want to divide the vehicle in parts (items).
\end{itemize}

When applying damage analysis on this item and checking the generalized asset list above, we would find that "Loosing the headlamp will drastically reduce the driver's sight and the veihcle's visability, which may result in a severe accident". This would mean that headlamp functionality is one of our primary assets (ISO-27005). We would also find that "Applying the headlamp at incorrect times could dazzle other vehicles, which may will increase the risk of an accident".
Then we would identify relevant security attributes for this primary asset and derive security goals as:
\begin{itemize}
    \item The integrity of the headlamp control functionality shall be preserved.
    \item The availability of the headlamp control functionality shall be preserved.
\end{itemize}

We would also claim (ISO-21434 definition of claim) that authenticity, non-repudiation, confidentiality and authority is not relevant for this primary asset. The item description, security goals and other non-functionality requirements will then be used at concept design. At concept design, a TARA will be performed on the item's primary assets using STRIDE that will result in cybersecurity requirements on certain components, which we will call supporting assets (ISO-27005). 
After that, attack path analyses are performed bottom-up, starting with some sort of attack library, for instance consisting of:
\begin{itemize}
    \item Intended over air connection (2,5G, 3G, 4G eller 5G, Wi-Fi, WPAN (Bluetooth, IrDA, Wireless USB, UBW, etc)
    \item Intended physical connection points (OBD, USB, CD-Rom, etc)
    \item Unintended Over-air disturbances (Radar, Laser, Electric Magnetic, microwaves, infrawaves, ultrasound, infrasound, etc)
    \item Unintended physical connection points (ECU, network, sensors, actuators, etc)
    \item ETC
\end{itemize}
The attack path analysis will verify that all supporting assets have been identified.
Then the component design will be started considering all requirements, including cybersecurity. The components and systems are then described in "product descriptions". The product descriptions are verified against the requirements, including cybersecurity. The components and systems are then tested against the product descriptions.

From this and your drawio picture, one security case structure would be:
\begin{itemize}
    \item Claim 0: Security of the realization of item (exterior lighting) is achieved.
Argument 0: Why Claim 0 is justified by claims 1-5.
    \item Claim 1 (Generic arguments): The performed work is adequate with respect to security.
    \item Claim 2 (White hat): Security goals covering all relevant security attributes of primary assets have been determined and assigned adequate impact levels (Operational, Safety, Legal \& Privacy and Financial). (Damage scenarios, asset identification, impact rating)
    \item Claim 3 (Black hat): Relevant supporting assets have been identified from analysis of threat agents, attacks (STRIDE) and attack paths. (Threat scenario identification, Attack path analysis).
    \item Claim 4 (Resolver): Adequate measures (resolvers) derived and implemented to fulfil the specified security goals considering the feasible attack paths. 
    \item Claim 5: Production, operation, service and decommissioning are all adequately handled.
    \item Claim 6: The product is maintained (and the cybersecurity case needs to be updated and re-evaluated when its assumptions e.g., threats, attacks, vulnerabilities, etc. are changed) throughout its lifetime.
\end{itemize}
	
The only difference I see from the assurance case example of ISO-21434 appendix G (and then your draw io picture), is that it starts with supporting assets rather than primary assets. The problem with this is, as I see it, is that the supporting assets are identified with the black hat rather than the white hat. That is when one understand the attack paths, it is possible to identify the supporting assets. So for the example I would say that the vehicle functionality “Control of vehicle headlamp” would be a primary asset.
Then, subclaims to claims 2-4 will be included in the evidence. That is, motivations (subclaims?) to claim 2 that the primary asset has been assigned the right impact level will be included in the damage scenarios. The motivations (subclaims) for claim 3 and 4 will be included in the TARA. Then the different verification and validation reports (work products of ISO-21434) will be the evidence for these claims.
However, when the case is generated, it will look similar to the draw io picture. Maybe claim 5 and 6 shall be included in the draw io picture also in some way? 

==> TexFiles/paperC/methodology.tex <==
\section{Methodology}\label{sec:method}
We used the following method to create and validate AD-SAC.
\begin{itemize}
    \item Create a high-level structure of an asset-driven SAC
    \item Extracted the relevant requirements and work products from ISO/SAE\,21434.
    \item Mapped the extracted items to the elements of AD-SAC
    \item Illustrate the approach using the example case from ISO/SAE\,21434.
    \item Validate the example case with experts from an industrial automotive OEM.
\end{itemize}
Each of the items 2-5 resulted in a revision of the approach and enhancements.

%To validate the approach, we considered the most valuable usage scenarios of SAC which we extracted in a previous work. These were:
%1. To assist decision makers in making go/no go decisions for products from a security perspective.
%2. To comply with security standards.

%For the first scenario, we created two cases. The first is based on an example case presented in ISO 21434, and the second is based on a case from the company. We created the cases together with two security experts from the case company (Örjan and Afshin). During this exercises, we made sure that the approach actually works and a case can be created based on it.....
%We made some variants of the cases, (by removing the CQ claims), and asked the participants to evaluate whether the cases are "good enough" to make go/no go decisions. We asked about their confidence in the cases as well.

%For the second scenario, we looked into the upcoming ISO standard, and made an exercise to map each requirement and work product of that standard to an element of the asset-driven approach. We (two researchers and one expert from the company) did this to make sure that the approach covers all the requirements in the standard. 
%We evaluated this with a compliance manager??





